Data-Driven System Level Synthesis

We establish data-driven versions of the System Level Synthesis (SLS) parameterization of achievable closed-loop system responses for a linear-time-invariant system over a finite-horizon. Inspired by recent work in data-driven control that leverages tools from behavioral theory, we show that optimization problems over system-responses can be posed using only libraries of past system trajectories, without explicitly identifying a system model. We first consider the idealized setting of noise free trajectories, and show an exact equivalence between traditional and data-driven SLS. We then show that in the case of a system driven by process noise, tools from robust SLS can be used to characterize the effects of noise on closed-loop performance, and further draw on tools from matrix concentration to show that a simple trajectory averaging technique can be used to mitigate these effects. We end with numerical experiments showing the soundness of our methods.

==> 00-abstract.tex <==

\begin{abstract}%
 An abstract would go here.%
\end{abstract}

==> 01-intro.tex <==
\section{Introduction}
\label{sec:intro}



\begin{itemize}
  \item Want to motivate this in terms of the DeePC work from Lygeros and Dorfler, as well as other model free work in LQR.
  \item First step towards providing rigorous theoretical understanding of robustness of noisy behavioral methods.
\end{itemize}




\red{Text block about Willems}
The work of Willems establishes the following:
a controllable linear dynamical system is completely determined
by its observed behavior on sufficiently ``exciting'' input~\cite{willems2005note}.
As a consequence, it is possible to
\emph{directly} parameterize the system dynamics from data.
In essence, this allows one to take a model-free approach to
the control of unknown systems:
rather than first estimating system dynamics via techniques such as
identify-then-control~\cite{dean2019sample},
the true underlying system is instead replaced by the data.
This enables end-to-end optimization without having to consider model quality.

This result has come to be known as the \emph{fundamental lemma of linear systems},
and is central to the study of data-driven control
~\cite{markovsky2005data, de2019persistency, tanzanakis2020data}.


\red{Text block about SLS}
System level synthesis~\cite{anderson2019system}
is a recent framework for the design and analysis of optimal optimal control.
At its core, SLS focuses on the \emph{system responses}
of a closed-loop linear dynamical system.
The power of this approach lies in the fact that problems such as
optimal LQR control now admit \emph{convex parameterizations},
and robust synthesis problems also have quasi-convex formulations.
This development has sparked a flurry of work
\red{cite all of Nik's publication over the last 5 years}.

Existing literature on SLS has an implicit assumption, however:
that either the underlying system \(A, B\) is known,
or that an estimation \(\tilde{A}, \tilde{B}\) is present
such that the spectral norm of the errors
\(\tilde{A} - A\) and \(\tilde{B} - B\) are small.
The former is the case when analyzing nominal dynamics;
while the latter is relevant for identify-then-control
data-driven approaches~\cite{dean2019sample}.
To the best of our knowledge, however,
no known works have investigated the usage of
direct data parameterization for SLS-based optimal robust control.

\paragraph{Notation} \red{To be updated, this is quickly copied/updated from my Robust MPC paper.  We will want to keep some of this though.}

We use $x_{[i:j]}$ as shorthand for the signal $[x^\top(i) \ x^\top(i+1) \ \cdots \ x^\top(j) ]^\top$.  For a signal $\sigma_{[0,T-1]}$, we define the Hankel matrix $\mcal{H}_L(\sigma_{[0,T-1]})$ of order $L$ to be:
\[
\mcal{H}_L (\sigma_{[0, T-1]})
            = \begin{bmatrix}
                \sigma(0) & \sigma(1) & \cdots & \sigma(T-L) \\
                \sigma(1) & \sigma(2) & \cdots & \sigma(T -L +1) \\
                \vdots & \vdots & \ddots & \vdots \\
                \sigma(L-1) & \sigma(L) & \cdots & \sigma(T - 1)
            \end{bmatrix}.
\]
A linear, causal operator $\mathbf{R}$ defined over a horizon of $T$ is represented by 
\begin{equation} \label{eq:BLT}
\mathbf{R} = \begin{bmatrix}
\dsuper{R}{0}{0} & \ & \ & \ \\
\dsuper{R}{1}{1} & \dsuper{R}{1}{0} & \ & \ \\
\vdots & \ddots & \ddots & \ \\
\dsuper{R}{T}{T} & \cdots & \dsuper{R}{T}{1} & \dsuper{R}{T}{0}
\end{bmatrix}
\end{equation} 
where $\dsuper{R}{i}{j} \in \mathbb{R}^{p \times q}$ is a matrix of compatible dimension. We denote the set of such matrices by $\mathcal{L}_{TV}^{T, p \times q}$ and will drop the superscript $T, p \times q$ when it is clear from the context. $\mathbf{R}(i,:)$ denotes the $i$-th block row of $\mathbf{R}$ and $\mathbf{R}(:,j)$ denotes the $j$-th block column of $\mathbf{R}$, both indexing from $0$.






==> 02-fund-lemma.tex <==
\section{Willems' Fundamental Lemma}
\label{sec:fund-lemma}

Willems' fundamental lemma is classically presented for
noiseless LTI systems of form
\begin{align}
    \label{eqn:lti-noiseless}
    z (t+1) = A z (t) + B u(t),
    \qquad z : \mbb{Z} \to \mbb{R}^n,
    \enskip u : \mbb{Z} \to \mbb{R}^m,
\end{align}
where the signals \(z, u\) are the state and control, respectively.
An extension to systems of form
\begin{align}
    \label{eqn:lti-noisy}
    x(t+1) = A x(t) + B u(t) + w(t),
    \qquad x, w : \mbb{Z} \to \mbb{R}^n,
    \enskip u : \mbb{Z} \to \mbb{R}^m
\end{align}
with random noise \(w\) is rather straightforward:
it suffices to incorporate \(w\) as an additional, albeit random,
component of the control.
What is of interest here is quantifying the effect of this perturbation:
this is necessary for the applying the robust SLS framework,
in which the quality of synthesized controllers decreases with noise.

Before proceeding we present some assumptions and notations
on \eqref{eqn:lti-noiseless} and \eqref{eqn:lti-noisy}.
First, the system matrices \(A, B\)
of \eqref{eqn:lti-noiseless} and \eqref{eqn:lti-noisy}
are assumed to be the same and also controllable.
The signals \(z, x\) are taken to be the states of
\eqref{eqn:lti-noiseless} and \eqref{eqn:lti-noisy}, respectively;
\(w\) the noise of \eqref{eqn:lti-noisy};
and \(u\) the control common to both ---
that is, \(u\) induces \(z\) while \(u, w\) induce \(x\).
Furthermore, signals are assumed to be zero for \(t < 0\) unless stated otherwise;
the indexing \(w(-1) = x(0) = z(0)\) is used for the initial condition.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Persistence of Excitation: Noiseless Case}
Central to Willems' fundamental lemma is
\emph{persistence of excitation},
which is classically presented as a rank condition on Hankel matrices
of the control input \(u\).

% \begin{definition}
%     \label{def:persistence}
%     Let \(\sigma : \mbb{Z} \to \mbb{R}^p\) be a signal.
%     We say that \(\sigma\) is persistently exciting of order
%     \(L\) if the Hankel matrix \(\mcal{H}_L (\sigma)\) has full rank, where
%     \begin{align*}
%         \mcal{H}_L (\sigma)
%             = \begin{bmatrix}
%                 \boldsymbol{\sigma}^{(0)}
%                     & \boldsymbol{\sigma}^{(1)}
%                     & \cdots
%                     & \boldsymbol{\sigma}^{(T - L)}
%                 \end{bmatrix}
%             = \begin{bmatrix}
%                 \sigma(0) & \sigma(1) & \cdots & \sigma(T-L) \\
%                 \sigma(1) & \sigma(2) & \cdots & \sigma(T -L +1) \\
%                 \vdots & \vdots & \ddots & \vdots \\
%                 \sigma(L-1) & \sigma(L) & \cdots & \sigma(T - 1)
%             \end{bmatrix}
%     \end{align*}
% \end{definition}

% \begin{definition}
%     \label{def:persistence}
%     Let \(\sigma : \mbb{Z} \to \mbb{R}^p\) be a signal.
%     We say that its finite-horizon restriction \(\sigma_{[0, T-1]}\)
%     is \emph{persistently exciting}
%     of order \(L\) if the Hankel matrix \(\mcal{H}_L (\sigma_{[0, T-1]})\) has full rank,
%     where
%     \begin{align*}
%         \sigma_{[0, T-1]}
%             = \begin{bmatrix}
%                 \sigma(0) \\ \sigma(1) \\ \vdots \\ \sigma(T - 1)
%                 \end{bmatrix},
%         \qquad
        
%     \end{align*}
% \end{definition}

The rank condition implies that \(T \geq (p + 1) L - 1\)
is a lower-bound on the horizon \(T\).
We assume that any Hankelized signal
\(\sigma\) has a sufficiently long horizon \(T\),
and therefore interchangeable use \(\sigma\)
and \(\sigma_{[0, T-1]}\) when context is clear.
Since different values of \(L\) alter both the height and width of \(\mcal{H}_{L} (\sigma)\),
if for \(L < L'\) two matrices \(\mcal{H}_L (\sigma)\) and \(\mcal{H}_{L'} (\sigma')\)
are stacked on top of each other,
then the right columns of \(\mcal{H}_L (\sigma)\) are dropped until
\(\begin{bmatrix} \mcal{H}_L (\sigma); \mcal{H}_{L'} (\sigma') \end{bmatrix}\)
is a rectangle.
As a convention, \(\mcal{H}_1 (\sigma)\) has \(T - L + 1\) columns.

In what follows we present Willem's fundamental lemma.

\begin{lemma}[Willems' Fundamental Lemma]
    \label{lem:fund-lemma00}
    Consider the system \eqref{eqn:lti-noiseless}
    with signals \(z, u\).
    If \(u\) is persistently exciting of order \(n + L\),
    then the following are true:
    \begin{enumerate}
        \item
        The following matrix has full rank \(= n + mL\)
        \begin{align*}
            \begin{bmatrix}
                \mcal{H}_1 (z) \\
                \mcal{H}_{L} (u)
            \end{bmatrix} =
            \begin{bmatrix}
                z(0) & z(1) & \cdots & z(T - L) \\
                \hline
                u(0) & u(1) & \cdots & u(T - L) \\
                \vdots & \vdots & \ddots & \vdots \\
                u(L - 1) & u(L) & \cdots & u(T - 1)
            \end{bmatrix}
        \end{align*}
        
        \item
        The signals
        \(z_{[0, L-1]} ^\star\) and \(u_{[0, L-1]} ^\star\)
        are valid length \(L\) trajectories of system \eqref{eqn:lti-noiseless}
        if and only if
        \begin{align*}
            \begin{bmatrix} z_{[0, L - 1]} ^\star \\ u_{[0, L - 1]} ^\star \end{bmatrix} =
            \begin{bmatrix} \mcal{H}_L (z) \\ \mcal{H}_L (u) \end{bmatrix} g,
            \qquad \text{for some \(g \in \mbb{R}^{T - L + 1}\)}
        \end{align*}
    \end{enumerate}
\end{lemma}
\begin{proof}
    See Appendix~\ref{sec:fund-lemma-proof}.
\end{proof}

Lemma~\ref{lem:fund-lemma} states that if the underlying system is controllable,
and \(\rank \mcal{H}_{n + L} (u) = n + L\),
then: (1) all initial conditions and inputs are parameterizable from observed signal data;
and (2) all valid trajectories are precisely the linear combinations of Hankelized data.
Most crucially, the underlying implication is that a linear dynamical system
is representable by its trajectory data --- provided the data is sufficiently rich.
Although consequential, this result is not altogether surprising given that
one of the underlying assumptions is controllability,
which is inherently a rank condition; indeed this is exploited in the proof.



% --- the implication is non-trivial.

% For one, this implies that a linear system can be \emph{represented} by its data:
% there is no need to explicitly estimate a model for \(A, B\) if the
% trajectory data is sufficiently rich.
% In the context of controller synthesis,
% the optimization problem is then directly formulated over the data,
% rather than over an estimated model as in identify-then-control schemes~\cite{dean2019sample}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Persistence of Excitation: Noisy Case}
Willems' lemma extends from \eqref{eqn:lti-noiseless} to \eqref{eqn:lti-noisy}
by appending \(w\) into the control signal.
In such a setting, Lemma~\ref{lem:fund-lemma} would
require \emph{both} \(u\) and \(w\)
to be persistently exciting of order \(L\);
the same results would then readily follow on this joint control input.

Although noise may be treated as part of the control,
there is an asymmetry in information:
Willem's lemma assumes the availability of \emph{all} control data,
whereas for \eqref{eqn:lti-noisy}
realistically only \(x, u\) are available while \(w\) is not.
This means that the Hankel matrices formed by
\(x, u\) will be \emph{slightly}
incorrect with respect to the equations in Lemma~\ref{lem:fund-lemma}.
For the purpose of analysis,
it is insightful to \emph{pretend}
that one has data of the \(w\) disturbance.
This assumption allows us to precisely analyze the
perturbation and deviation of trajectory data
from a noisy system \eqref{eqn:lti-noisy}
in contrast with a noiseless one \eqref{eqn:lti-noiseless}.
Furthermore, if one knows apriori that,
for instance \(w(t) \sim \mcal{N}(0, \sigma^2 I)\),
then concentration bounds readily follow.

\begin{lemma}
    \label{lem:noisy-hankel-dynamics}
    Let signals \(z, x\) be the states for
    systems \eqref{eqn:lti-noiseless}, \eqref{eqn:lti-noisy},
    respectively, driven by \(u\) and \(w\).
    Suppose \(u\) and \(w\) are both persistently exciting of order \(n + L\),
    then it holds that
    \begin{align*}
        \mcal{H}_L (x)
        =
        \mcal{H}_L (z)
        + \mcal{T}_L (I) \mcal{H}_L (w)
        + \mcal{O}_L (A) \mcal{W}_{[0, T - L]}
    \end{align*}
    where \(\mcal{W}(t) = \sum_{k = 0}^{t - 1} A^{t - 1 - k} w(k)\)
    are columns of  
    \(\mcal{W}_{[0, T-L]}
            = \begin{bmatrix} \mcal{W}(0) & \cdots & \mcal{W}(T - L) \end{bmatrix}\),\footnote{We let $\mathcal{W}(0) = 0$ by convention.}
    and
    \begin{align*}
        \mcal{O}_L (X)
            = \begin{bmatrix}
                I \\ X \\ \vdots \\ X^{L-1}
            \end{bmatrix},
        \qquad
        \mcal{T}_L (X)
            = \begin{bmatrix}
                    0 \\
                    X & 0 \\
                    AX & X & \ddots \\
                    \vdots & \vdots & \ddots & \ddots \\
                    A^{L - 2} & A^{L - 3} & \cdots & X & 0
                \end{bmatrix}
    \end{align*}
    
\end{lemma}
\begin{proof}
    Let \(z_{[t, t-L+1]}\) and \(x_{[t, t+L-1]}\)
    be an arbitrary pair of columns of \(\mcal{H}_L (z)\) and \(\mcal{H}_L (x)\).
    Then
    \begin{align*}
        z_{[t, t + L - 1]}
            &= \mcal{O}_L (A) z(t) + \mcal{T}_L (B) u_{[t, t + L - 1]} \\
        x_{[t, t + L - 1]}
            &= \mcal{O}_L (A) x(t) + \mcal{T}_L (B) u_{[t, t+L-1]} + \mcal{T}_L (I) w_{[t, t+L-1]}
    \end{align*}
    by the dynamics of
    \eqref{eqn:lti-noiseless} for the first line
    and \eqref{eqn:lti-noisy} for the second.
    Since \(z(0) = x(0)\),
    using the same control sequence \(u\) on both systems reveals
    the perturbation factor \(x(t) = z(t) + \mcal{W}(t)\).
    Consequently,
    \begin{align*}
        x_{[t, t + L - 1]}
            &= \mcal{O}_L (A) (z(t) + \mcal{W}(t)) + \mcal{T}_L (B) u_{[t, t+L-1]} + \mcal{T}_L (I) w_{[t, t+L-1]}
    \end{align*}
    Extending this to all columns of the Hankel matrices completes the proof.
\end{proof}

Another form of \(\mcal{W}_{[0, T-L]}\) is this:
let \(U_L \in \mbb{R}^{L \times L}\) be the upper-triangular matrix of all \(1\)'s,
then
\begin{align*}
    \mcal{W}_{[0, T-L]}
        = \begin{bmatrix} I_n & 0 & \cdots & 0 \end{bmatrix}
            \mcal{H}_L (w)
            (U_L \otimes I_n)
\end{align*}
Our primary interest for the decomposition in Lemma~\ref{lem:noisy-hankel-dynamics}
is sub-optimality analysis:
by comparing the performance of a controller synthesized on noisy data \(x, u\)
to one derived from noiseless data \(z, u\),
we can precisely analyze the effect of noise on optimal controller synthesis.


% \begin{lemma}
%     \label{lem:willems-noisy-perturb}
%     Suppose that \(z, u\) is noiseless data
%     from system~\eqref{eqn:lti-noiseless} on which
%     \begin{align*}
%         \begin{bmatrix}
%             \bar{z}_{[0, L - 1]} \\ \bar{u}_{[0, L - 1]}
%         \end{bmatrix} =
%         \begin{bmatrix}
%             \mcal{H}_L (z) \\
%             \mcal{H}_L (u)
%         \end{bmatrix} g,
%         \qquad \text{for some \(g \in \mbb{R}^{T - L + 1}\)}
%     \end{align*}
%     If process noise \(w\) perturbs the system
%     and \(u\) is independent of \(w\),
%     then this \(g\) will induce on noisy state data
%     \begin{align*}
%         \bar{x}_{[0, L - 1]}
%         = \bar{z}_{[0, L-1]}
%             + \mcal{T}_L (I) \mcal{H}_L (w) g
%             + \mcal{O}_L (A)
%                 \mcal{W}_{[0, T-L]}
%                 g
%     \end{align*}
% \end{lemma}
% \begin{proof}    
%     \red{AAAAAAAAAAAAAAAAAAAAAAA}
% \end{proof}



==> 03-data-driven-sls.tex <==
\section{Data-Driven System Level Synthesis}
\label{sec:data-sls}

% In this section we present a data-parameterized approach to SLS.
% We begin with a tutorial on SLS:
% a more extensive introduction can be found in~\cite{anderson2019system}.
% Next, we build up towards constructing system response matrices
% by analyzing the case of no noise, and then later incorporating noise.
% Finally, we formulate the data-parameterized robust SLS LQR problem.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{A Quick Tutorial on System Level Synthesis}
% Consider an \(L\)-length trajectory from system~\eqref{eqn:lti-noisy}
% expressed as block matrix operations
% \begin{align}
%     \label{eqn:stacked-dynamics}
%     x_{[0, L-1]}
%         = \mcal{Z} \mcal{A} x_{[0, L-1]}
%             + \mcal{Z} \mcal{B} u_{[0, L-1]}
%             + w_{[-1, L-2]}
% \end{align}
% where \(\mcal{A} = I_L \otimes A\),
% and \(\mcal{B} = I_L \otimes B\),
% and where \(\mcal{Z}\) is the block-downshift operator.
% If it is also the case that the system~\eqref{eqn:stacked-dynamics}
% satisfies the linear feedback control law
% \(u_{[0, L-1]} = \mcal{K} x_{[0, L-1]}\)
% where \(\mcal{K}\) is a block-lower-triangular matrix,
% then rewriting \eqref{eqn:stacked-dynamics} we arrive at
% \begin{align*}
%     x_{[0, L-1]}
%         &= (I - \mcal{Z} (\mcal{A} + \mcal{B} \mcal{K}))^{-1} w_{[-1, L-2]}
%         = \Phi_x w_{[-1, L-2]}
%         \\
%     u_{[0, L-1]}
%         &= \mcal{K} (I - \mcal{Z} (\mcal{A} + \mcal{B} \mcal{K}))^{-1} w_{[-1, L-2]}
%         = \Phi_u w_{[-1, L-2]}
% \end{align*}
% which captures how the process noise \(w\)
% maps to the state \(x\) and control \(u\).
% \(\Phi_x, \Phi_u\) are known as the \emph{system response} matrices,
% which are block-lower-triangular matrices that map noise to state and controls respectively.
% The parameterization of system responses
% and their relation to linear feedback controllers is summarized
% in the theorem below.

% \begin{theorem}
%     \label{thm:sls-thm}
%     For a system~\eqref{eqn:lti-noisy}
%     with block-lower-triangular state feedback over horizon \(L\),
%     with action \(u_{[0, L-1]} = \mcal{K} x_{[0, L-1]}\),
%     the following are true
%     \begin{enumerate}
%         \item The affine subspace defined by
%         \begin{align}
%             \label{eqn:sls-constr}
%             \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & -\mcal{Z} \mcal{B} \end{bmatrix}
%             \begin{bmatrix} \Phi_x \\ \Phi_u \end{bmatrix}
%             = I
%         \end{align}
%         parameterizes all possible system responses from \(w\) to \(x\) and \(u\).
    
%         \item For any block-lower-triangular matrices \(\Phi_x, \Phi_u\)
%         satisfying \eqref{eqn:sls-constr},
%         the controller \(\mcal{K} = \Phi_u \Phi_x ^{-1}\)
%         achieves the desired response.
%     \end{enumerate}
    
% \end{theorem}
% \begin{proof}
%     See \cite{anderson2019system} Theorem 2.1.
% \end{proof}

% In addition to both \(\Phi_x, \Phi_u\) being block-lower-triangular,
% the constraint \eqref{eqn:sls-constr} additionally implies that
% \(\Phi_x\) has identities along its block diagonal.
% The block-lower-triangular structure ensures \emph{causality}:
% the signals \(w(t), u(t)\) are not functions of
% future noise \(w(s)\) where \(s > t\).

% A key strength of SLS is that the parameterization of \(\Phi_x, \Phi_u\)
% is affine, and therefore convex.
% Consequently, the search for an optimal feedback control law
% is also reduced to a convex problem:
% rather than searching directly for the controller \(\mcal{K}\),
% it suffices to search for the system responses.
% Furthermore, a number of problems gain convexity for free.
% In particular, we are interested in the stochastic LQR problem
% with \(w(t) \sim \mcal{N}(0, \sigma^2 I)\),
% \begin{align}
%     \label{eqn:lqr}
%     \minimize_{x, u}
%         \enskip
%         \E_w \bracks{\sum_{t = 0}^{L - 1} x(t) ^\top Q x(t) + u(t) ^\top R u(t)}
%         \qquad \text{subject to \eqref{eqn:stacked-dynamics}}
% \end{align}
% where \(Q \succeq 0\) (positive semi-definite) and \(R \succ 0\) (positive definite).
% Under an SLS re-parameterization, this is written as
% \begin{align}
%     \label{eqn:sls-lqr}
%     \minimize_{\Phi_x, \Phi_u}
%         \enskip
%         \sigma
%         \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
%                     \begin{bmatrix} \Phi_x \\ \Phi_u \end{bmatrix}}_F
%     \qquad \text{subject to \eqref{eqn:sls-constr}}
% \end{align}
% where \(\mcal{Q} = I_L \otimes Q\) and \(\mcal{R} = I_L \otimes R\).
% A derivation is given in Section 2.2 of \cite{anderson2019system}.
% % As \(\mcal{K} = \Phi_u \Phi_x ^{-1}\) is causal (block lower-triangular),
% % the linear feedback control law then takes on several equivalent forms
% % \begin{align*}
% %     u(t) = \sum_{k = 0}^{t} \Phi_u (t, t - k) w(k)
% %         = \sum_{k = 0}^{t} \mcal{K} (t, t-k) x(k)
% %         = \sum_{k = 0}^{t} (\mcal{K} \Phi_x)(t, t-k) w(k)
% % \end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Noiseless Data Parameterization}
Suppose that \(w(t) = 0\) for all \(t \geq 0\),
the system response matrices then simplify to


% For notation we opt to use \(x\) rather than \(z\) like earlier
% as this makes presentation smoother.

% Classically SLS assumes the availability of the system matrices \(A, B\),
% and if not, then estimates of \(\hat{A}, \hat{B}\).
% In what follows, we analyze the scenario where one does \emph{not}
% use \(A, B\) --- or an estimate --- to synthesize a controller.
% As a simplification, our initial analysis focuses on
% the case of where system~\eqref{eqn:lti-noisy} lacks process noise.
% As an indexing trick, we express this as
% \(w(-1) = x(0)\), and \(w(t) = 0\) for all other \(t \neq -1\).
% Because we only need care about the initial disturbance,
% the system response matrices simplify to
\begin{align*}
    x_{[0, L-1]}
        = \Phi_x \begin{bmatrix} x(0) \\ 0 \\ \vdots \\ 0 \end{bmatrix}
        = \Phi_x (:, 0) x(0),
    \qquad
    u_{[0, L-1]}
        = \Phi_u \begin{bmatrix} x(0) \\ 0 \\ \vdots \\ 0 \end{bmatrix}
        = \Phi_u (:, 0) x(0)
\end{align*}
Here the first-block columns \(\Phi_x (:, 0), \Phi_u (:, 0)\)
map the initial condition \(w(-1) = x(0)\)
to system trajectories of \(x, u\) respectively.
Since only the first block-column is affected by disturbance,
the affine constraint~\eqref{eqn:sls-constr} therefore reduces to
\begin{align}
    \label{eqn:noiseless-sls-constr0}
    \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & -\mcal{Z} \mcal{B} \end{bmatrix}
    \begin{bmatrix} \Phi_x (:, 0) \\ \Phi_u (:, 0) \end{bmatrix}
    = \begin{bmatrix} I  \\ 0 \\ \vdots \\ 0 \end{bmatrix}
\end{align}
and likewise the noise-to-trajectory semantics of the system
response matrices mean that
\begin{align*}
    \bigg\{
        \begin{bmatrix} \Phi_x (:, 0) \\ \Phi_u (:, 0) \end{bmatrix}
        : \text{maps \(x(0)\) to}
            \,
            \begin{bmatrix} x_{[0, L-1]} \\ u_{[0, L-1]} \end{bmatrix}
            \,
            \text{for \(A, B\)}
    \bigg\}
    =
    \bigg\{
    \begin{bmatrix} \Phi_x (:, 0) \\ \Phi_u (:, 0) \end{bmatrix}
        : \text{satisfies \eqref{eqn:noiseless-sls-constr}}
    \bigg\}
\end{align*}
In other words, the first block-columns \(\Phi_x (:, 0), \Phi_u (:, 0)\)
that map \(x(0)\) to valid trajectories
are precisely those that satisfy \eqref{eqn:noiseless-sls-constr}.
This connection allows us to formally relate
the first block of system response matrices
to parameterizations with persistently exciting data.
%% rough notes on how to transition from SLS to data driven
%Our approach to connecting the SLS parameterization of Theorem 4 to the fundamental theorem described in Lemma 2 is to observe that the i-th column of Phi_x and Phi_u correspond to the impulse response of the closed loop system to the i-th disturbance element w_i.  Thus it suffices to constrain the free variable in Lemma 2 such that the resulting system trajectory is one induced by an impulse.
% \begin{theorem}
% %% this is super clumsy, why not just use the noiseless system for this part.  We'll discuss, but I think we should reorg and do everything noise free first.
    
%     Consider the system \eqref{eqn:lti-noisy} with
%     \(u\) persistently exciting of order \(n + L\).
%     If perturbance occurs only at the initial condition \(w(-1) = x(0)\),
%     then
%     \begin{align*}
%         \bigg\{\begin{bmatrix} \Phi_x (:, 0) \\ \Phi_u (:, 0) \end{bmatrix}
%             : \text{satisfies \eqref{eqn:noiseless-sls-constr}}
%         \bigg\}
%         =
%         \bigg\{
%             \begin{bmatrix}
%                 \mcal{H}_L (x) \\ \mcal{H}_L (u)
%             \end{bmatrix}
%             G
%             : G \in \Gamma (x)
%         \bigg\},
%     \end{align*}
%     where \(\Gamma (x) = \{G : \mcal{H}_1 (x) G = I\}\).
% \end{theorem}
% \begin{proof}
% For ease of notation, define
% \(\Phi(:,0) = \begin{bmatrix} \Phi_x (:,0) ; \Phi_u (:,0) \end{bmatrix}\).
% Additionally, call the left and right-hand sets as LHS and RHS respectively.


% (\(\subseteq\))
% Consider some \(\Phi(:,0) \in \mrm{LHS}\).
% Because \(u\) is persistently exciting of order \(n + L\),
% it is also persistently exciting of order \(L\).
% With Lemma~\ref{lem:fund-lemma} this implies that
% \begin{align*}
%     \braces{ \begin{bmatrix} x_{[0, L-1]} ^\star \\ u_{[0,L-1]} ^\star \end{bmatrix}
%             : \text{valid trajectories of \(A, B\)}}
%     = \braces{\begin{bmatrix} \mcal{H}_L (x) \\ \mcal{H}_L (u) \end{bmatrix} g,
%         g \in \mbb{R}^{T - L + 1}}
% \end{align*}
% Since the matrices \(\Phi(:,0)\) are precisely the ones that generate
% valid trajectories of \(A, B\) from an initial state,
% it is also the case that
% \begin{align*}
%     \mrm{span} (\mrm{LHS}) =
%         \braces{ \begin{bmatrix} x_{[0, L-1]} ^\star \\ u_{[0,L-1]} ^\star \end{bmatrix}
%             : \text{valid trajectories of \(A, B\)}}
% \end{align*}
% In other words, every column of \(\Phi(:,0) \in \mrm{LHS}\) is in the range of
% the stacked data block Hankel matrix.
% That is, there exists \(g_1, g_2, \ldots, g_n\) such that:
% \begin{align*}
%     \Phi(:,0)
%         = \begin{bmatrix}
%             | & | & \cdots & | \\
%             \phi_1 & \phi_2 & \cdots & \phi_n \\
%             | & | & \cdots & |
%             \end{bmatrix}
%         = \begin{bmatrix}
%             \mcal{H}_L (x) \\ \mcal{H}_L (u)
%             \end{bmatrix}
%             \begin{bmatrix}
%             | & | & \cdots & | \\
%             g_1 & g_2 & \cdots & g_n \\
%             | & | & \cdots & |
%             \end{bmatrix}
%         = \begin{bmatrix}
%             \mcal{H}_L (x) \\ \mcal{H}_L (u)
%             \end{bmatrix}
%             G
% \end{align*}
% Note that \(\Phi_x (0,0) = I\),
% because the output trajectory of \(\Phi_x (:,0) x^\star (0)\)
% includes \(x^\star (0)\) as its first block.
% Furthermore, since \(\mcal{H}_1 (x)\)
% is the first block row of \(\mcal{H}_L (x)\)
% and its right-multiplication by \(G\) equals \(I\),
% it follows that \(G \in \Gamma(x)\).
% Conclude that \(\mrm{LHS} \subseteq \mrm{RHS}\).


% (\(\supseteq\))
% Consider a \(\Phi(:,0) \in \mrm{RHS}\).
% Substituting this into the LHS' constraint:
% \begin{align*}
%     \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & - \mcal{Z} \mcal{B} \end{bmatrix}
%     \begin{bmatrix} \Phi_x (:,0) \\ \Phi_u (:,0) \end{bmatrix}
%     = \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & - \mcal{Z} \mcal{B} \end{bmatrix}
%         \begin{bmatrix} \mcal{H}_L (x) \\ \mcal{H}_L (u) \end{bmatrix} G
%     = \begin{bmatrix} \mcal{H}_1 (x) \\ 0 \end{bmatrix} G
% \end{align*}
% where we invoke \eqref{eqn:data-only-constr} with \(\mcal{H}_L (w) = 0\).
% Since \(\mcal{H}_1 G = I\) by definition of \(G \in \Gamma(x)\),
% \begin{align*}
%     \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & - \mcal{Z} \mcal{B} \end{bmatrix}
%     \begin{bmatrix} \Phi_x (:,0) \\ \Phi_u (:,0) \end{bmatrix}
%     = \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & - \mcal{Z} \mcal{B} \end{bmatrix}
%         \begin{bmatrix} \mcal{H}_L (x) \\ \mcal{H}_L (u) \end{bmatrix} G
%     = \begin{bmatrix} I \\ 0 \\ \vdots \\ 0 \end{bmatrix}
% \end{align*}
% Conclude that \(\mrm{LHS} \supseteq \mrm{RHS}\).
% \end{proof}
% Theorem~\ref{thm:noiseless-data-sls}
% gives the condition under which \(x, u\)
% precisely parameterizes the \(\Phi_x (:, 0)\) and \(\Phi_u (:, 0)\)
% for systems where process noise affects only the initial condition.
% For a controllable \(A, B\) and a sufficiently exciting \(u\),
% the problem of controller design then reduces to finding a \(G \in \Gamma (x)\)
% to shape how \(\Phi_x (:, 0)\) and \(\Phi_u (:, 0)\)
% will map any initial condition.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Noisy Data Parameterization}
We now turn our attention to the case when \(w\) is no longer zero.
The goal here is to employ robust control techniques from SLS
to synthesize controllers in a principle manner in the presence of random noise.
In this case, the system response matrices \(\hat{\Phi}_x, \hat{\Phi}_u\)
synthesized from noisy data may not precisely satisfy \eqref{eqn:sls-constr}.

% \begin{theorem}
%     \label{thm:robust-sls}
%     Let \(\Delta\) be a strictly block-lower-triangular matrix,
%     and suppose \(\hat{\Phi}_x, \hat{\Phi}_u\)
%     are \emph{approximately} system responses to \eqref{eqn:lti-noisy}
%     which satisfy
%     \begin{align}
%         \label{eqn:approx-sls-constr}
%         \begin{bmatrix}
%             (I - \mcal{Z} \mcal{A}) & -\mcal{Z} \mcal{B}
%         \end{bmatrix}
%         \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}
%         = I + \Delta
%     \end{align}
%     If \((I + \Delta)^{-1}\) exists,
%     then the controller \(\hat{\mcal{K}} = \hat{\Phi}_u \hat{\Phi}_x ^{-1}\)
%     achieves for the true system~\eqref{eqn:lti-noisy} the behavior of
%     \(\hat{\Phi}_x (I + \Delta)^{-1} : w \mapsto x\) and
%     \(\hat{\Phi}_u (I + \Delta)^{-1} : w \mapsto u\).
% \end{theorem}
% \begin{proof}
%     See \cite{anderson2019system} Theorem 2.2.
% \end{proof}

% The challenge now is to formulate a block-square matrices
% \(\hat{\Phi}_x, \hat{\Phi}_u\)
% from data alone.
% Our approach involves first synthesizing the block-columns of
% \(\hat{\Phi}_x, \hat{\Phi}_u\),
% before combining them into the final result.
% For data, although we have access to only \(x, u\),
% it is instructive to also consider \(w\) in the analysis.
% To begin, since each column of
% \(\mcal{H}_L (x), \mcal{H}_L (u), \mcal{H}_L (w)\)
% satisfies~\eqref{eqn:stacked-dynamics},
% it follows that
% \begin{align}
%     \label{eqn:data-only-constr}
%     \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & -\mcal{Z} \mcal{B} \end{bmatrix}
%     \begin{bmatrix} \mcal{H}_L (x) \\ \mcal{H}_L (u) \end{bmatrix}
%     =
%     \begin{bmatrix} \mcal{H}_1 (x) \\ 0 \end{bmatrix}
%     + \mcal{Z} \mcal{H}_L (w)
% \end{align}
% Using some \(\hat{G} \in \Gamma (x)\)
% such that \(\hat{\Phi}_x (:, 0) = \mcal{H}_L (x) \hat{G}\)
% and \(\hat{\Phi}_u (:, 0) = \mcal{H}_L (u) \hat{G}\)
% as in Lemma~\ref{thm:noiseless-data-sls},
% \begin{align}
%     \label{eqn:one-col-constr}
%     \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & -\mcal{Z} \mcal{B} \end{bmatrix}
%     \begin{bmatrix} \hat{\Phi}_x (:, 0) \\ \hat{\Phi}_u (:, 0) \end{bmatrix}
%     =
%     \begin{bmatrix} I \\ 0 \\ \vdots \\ 0 \end{bmatrix}
%     + \underbrace{\mcal{Z} \mcal{H}_L (w) \hat{G}}_{``\Delta"}
% \end{align}
% Modulo down-shifting, \eqref{eqn:one-col-constr}
% demonstrates the construction of a single block-column of
% \(\hat{\Phi}_x, \hat{\Phi}_u\).
% This bears strong resemblance to \eqref{eqn:noiseless-sls-constr},
% and indeed examining \eqref{eqn:approx-sls-constr}
% one expects a ``\(\Delta\)'' term to appear for approximate system responses;
% in this case it is \(\mcal{Z} \mcal{H}_L (w) G\).

% The construction of the other columns is similar;
% in general consider
% \(\hat{G}_0, \ldots, \hat{G}_{L - 1} \in \Gamma(x)\),
% where each \(\hat{G}_{k - 1}\) is used to construct the \(k\)th column of
% \(\hat{\Phi}_x, \hat{\Phi}_u\).
% Since \(\mcal{Z}\) commutes with block-diagonal matrices,
% with shifting the \(k\)th column is then
% \begin{align}
%     \label{eqn:k-col-constr}
%     \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & -\mcal{Z} \mcal{B} \end{bmatrix}
%     \begin{bmatrix}
%         \mcal{Z}^{k - 1} \mcal{H}_L (x) \\
%         \mcal{Z}^{k - 1} \mcal{H}_L (u)
%     \end{bmatrix}
%     \hat{G}_{k - 1}
%     = \mcal{Z}^{k - 1} \begin{bmatrix} I \\ 0 \\ \vdots \\ 0 \end{bmatrix}
%         + \mcal{Z}^k \mcal{H}_L (w) \hat{G}_{k - 1}
% \end{align}
% This idea is formalized as follows.

% \begin{theorem}
%     \label{thm:noisy-data-sls}
%     For a system~\eqref{eqn:lti-noisy}
%     with \(u, w\) both persistently exciting of order \(n + L\),
%     the approximate system response matrices and \(\Delta\) are given by
%     \begin{align}
%         \hat{\Phi}_x
%             &= \mcal{O}_L (\mcal{Z}^\top)^\top
%                 (I_L \otimes \mcal{H}_L (x)) \hat{\mcal{G}}
%                 \label{eqn:hat-phix} \\
%         \hat{\Phi}_u
%             &= \mcal{O}_L (\mcal{Z}^\top)^\top
%                 (I_L \otimes \mcal{H}_L (u)) \hat{\mcal{G}}
%                 \label{eqn:hat-phiu} \\
%         \Delta
%             &= \mcal{O}_L (\mcal{Z}^\top)^\top
%                 (I_L \otimes \mcal{Z} \mcal{H}_L (w))
%                 \hat{\mcal{G}}
%             \label{eqn:delta}
%     \end{align}
%     where
%     \(\mcal{O}_L (\mcal{Z}^\top)^\top
%         = \begin{bmatrix} I & \mcal{Z} & \cdots & \mcal{Z}^{L - 1} \end{bmatrix}\)
%     and
%     \(\hat{\mcal{G}}\) is block-lower-triangular of form
%     \begin{align}
%         \hat{\mcal{G}}
%             = \begin{bmatrix}
%                 \hat{G}_0 \\
%                 \star & G_1 \\
%                 \vdots & \vdots & \ddots \\
%                 \star & \star & \cdots & \hat{G}_{L - 1}
%               \end{bmatrix},
%                 \qquad
%                 \hat{G}_0, \ldots, \hat{G}_{L - 1} \in \Gamma(x)
%         \label{eqn:mcalG}
%     \end{align}
% \end{theorem}
% \begin{proof}
%     It follows from the block dynamics of \eqref{eqn:data-only-constr} that
%     \begin{align*}
%         \begin{bmatrix} (I - \mcal{Z} \mcal{A}) & -\mcal{Z} \mcal{B} \end{bmatrix}
%         \begin{bmatrix}
%             \mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{H}_L (x)) \\
%             \mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{H}_L (u))
%         \end{bmatrix}
%         = 
%         \mcal{O}_L (\mcal{Z}^\top)^\top
%         \parens{I_L \otimes
%             \parens{\begin{bmatrix} \mcal{H}_1 (x) \\ 0 \end{bmatrix} + \mcal{Z} \mcal{H}_L (w)}}
%     \end{align*}
%     Here \(\mcal{Z}\)
%     commutes with \(\mcal{A}\) and \(\mcal{B}\)
%     (adjusting for dimensions of right-multiplication)
%     because \(\mcal{A}\) and \(\mcal{B}\) are block-diagonal matrices with
%     repeated diagonal blocks.
%     Therefore, the action of \(\mcal{Z}\) during left-multiplication (down-shifting)
%     and right-multiplication (left-shifting)
%     produce the same effect.
    
%     %% need to specify that [I-ZA, -ZB] commutes with O_L because of LTI system and banded structure.
%     Consider \(\hat{G}_0, \ldots, \hat{G}_{L - 1} \in \Gamma(x)\)
%     that forms \(\hat{\mcal{G}}\) with arbitrary elements below the block diagonal.
%     Right-multiplying by \(\hat{\mcal{G}}\) on both sides,
%     the RHS yields
%     \begin{align*}
%         \mcal{O}_L (\mcal{Z}^\top)^\top
%         \parens{I_L \otimes \begin{bmatrix} \mcal{H}_1 (x) \\ 0 \end{bmatrix}} \mcal{G}
%         = I_{nL}
%     \end{align*}
%     and \(\mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{Z} \mcal{H}_L (w))\)
%     is strictly block-lower triangular.
%     As such, the RHS has form \(I + \Delta\).
%     Furthermore, since \(\mcal{O}_L (\mcal{Z}^\top)^\top\)
%     and \(\hat{\mcal{G}}\)
%     are both block-lower-triangular,
%     conclude that both \(\hat{\Phi}_x, \hat{\Phi}_u\) are too.
%     Not only this, the diagonal entries of \(\hat{\Phi}_x\) are the identity,
%     and so \(\hat{\Phi}_x, \hat{\Phi}_u\)
%     are valid approximate system responses.
% \end{proof}

% Theorem~\ref{thm:noisy-data-sls} states the parameterization
% of approximate system response matrices \(\hat{\Phi}_x, \hat{\Phi}_u\)
% in terms of the data of \(x, u\).
% With \(\Delta \neq 0\), Theorem~\ref{thm:robust-sls} also applies:
% the system response induced by \(\hat{\mcal{K}} = \hat{\Phi}_u \hat{\Phi}_x ^{-1}\)
% will yield
% \(\hat{\Phi}_x (I + \Delta)^{-1} : w \mapsto x\)
% and \(\hat{\Phi}_u (I + \Delta)^{-1} : w \mapsto u\).
% Consequently, the optimal stochastic LQR cost of using a controller \(\hat{K}\)
% synthesized on noisy data with each \(w(t) \sim \mcal{N}(0, \sigma^2 I)\)
% can be cast as the optimization problem
% \begin{align}
%     \label{eqn:noisy-data-sls-lqr}
%     \minimize_{\hat{\mcal{G}}}
%         &\quad
%             \sigma
%             \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
%             \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}
%             (I + \Delta)^{-1}}_F \\
%     \text{subject to}
%         &\quad
%             \text{\eqref{eqn:hat-phix}, \eqref{eqn:hat-phiu}, \eqref{eqn:delta}, \eqref{eqn:mcalG}}
%     \nonumber
% \end{align}
% This is a non-convex problem because
% \(\Delta\) depends linearly on \(\hat{\mcal{G}}\).
% However, we formulate and analyze a data-independent convex upper-bound.
% Using the inequality
% \(\norm{M_1 M_2}_F \leq \norm{M_1}_F \cdot \norm{M_2}_2\),
% the objective of \eqref{eqn:noisy-data-sls-lqr} is upper-bounded via
% \begin{align*}
%     \sigma \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
%             \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}
%             (I + \Delta)^{-1}}_F
%     &\leq
%     \sigma
%     \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
%     \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}}_F
%     \cdot \norm{(I + \Delta)^{-1}}_2\\
%     &\leq \frac{\sigma}{1 - \gamma}
%         \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
%         \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}}_F
% \end{align*}
% provided that \(\norm{\Delta}_2 \leq \gamma < 1\).
% This allows us to write the robust control problem as
% \begin{align}
%     \label{eqn:robust-data-sls-lqr}
%     \minimize_{\gamma \in [0, 1), \, \hat{\mcal{G}}}
%         &\quad
%             \frac{\sigma}{1 - \gamma}
%             \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
%             \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}}_F \\
%     \text{subject to}
%         &\quad \text{\eqref{eqn:hat-phix}, \eqref{eqn:hat-phiu}, \eqref{eqn:delta}, \eqref{eqn:mcalG}} \nonumber \\
%         &\quad \norm{\Delta}_2 \leq \gamma \nonumber
%     \nonumber
% \end{align}
% which is quasi-convex in \(\gamma\) and convex in \(\hat{\mcal{G}}\).





==> 04-sub-opt.tex <==
\section{Sub-optimality Analysis}
\label{sec:opt-control}

In this section we analyze the sub-optimality of
using a robust controller
\(\hat{\mathcal{K}} = \hat{\Phi}_u \hat{\Phi}_x ^{-1}\)
for the stochastic LQR problem.
The goal is to compare the performance of this robust
controller against
an optimal controller \(\mathcal{K}^\star\)
synthesized from data \emph{without} noise.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
    \label{lem:feas-soln}
    Suppose that \(\norm{\mcal{H}_L (w)}_2 \leq \varepsilon < 1 / L^2\)
    and each \(w(t) \sim \mcal{N}(0, \sigma^2 I)\).
    Define
    \begin{align*}
        \mcal{G}^\star
        = \begin{bmatrix}
            G_0 ^\star \\
            \star & G_1 ^\star \\
            \vdots & \vdots & \ddots \\
            \star & \star & \cdots & G_{L - 1} ^\star
        \end{bmatrix},
        \qquad
        G_0 ^\star, \ldots, G_{L - 1} ^\star \in \Gamma(z)
    \end{align*}
    where \(\mcal{G}^\star\) is optimal LQR solution
    synthesized from noiseless data \(z, u\).
    If the following norm bounds are satisfied
    \begin{align*}
        \norm{\mcal{G}^\star}_2 < \frac{\sqrt{L} (1 - \sqrt{\varepsilon})}{\sqrt{\varepsilon}},
        \qquad
        \norm{G_k ^\star}_2 \leq \frac{\pi}{\sqrt{\varepsilon} (2 L + \log L)}
        \quad \text{for} \enskip 0 \leq k \leq L - 1
    \end{align*}
    then \(\mcal{G}_0 = \mcal{G}^\star (I + \mcal{D})^{-1}\)
    with \(\gamma_0 = \sqrt{\varepsilon} L\)
    is a feasible for \eqref{eqn:robust-data-sls-lqr}
    where
    \begin{align*}
        \mcal{D} = \trm{diag}(D_0, \ldots, D_{L - 1}),
        \qquad
        D_k = \mcal{W}_{[0, T-L]} G_k ^\star
        \quad \text{for} \enskip 0 \leq k \leq L - 1
    \end{align*}
\end{lemma}
\begin{proof}
    We first show that the algebraic relations are satisfied
    before proving the norm constraint required of \eqref{eqn:robust-data-sls-lqr}.
    First, the relation \(\mcal{H}_1 (x) = \mcal{H}_1 (z) + \mcal{W}_{[0, T-L]}\)
    follows from Lemma~\ref{lem:noisy-hankel-dynamics}
    as the top block of \(\mcal{T}_L (I) \mcal{H}_L (w)\) is zero
    and the top block of \(\mcal{O}_L (A)\) is \(I\),
    so multiplying by any \(G_k ^\star\) yields
    \begin{align*}
        \mcal{H}_1 (x) G_k ^\star
        = \mcal{H}_1 (z) G_k ^\star + \mcal{W}_{[0, T-L]} G_k ^\star
        = I + D_k
    \end{align*}
    This implies that \(G_k (I + D_k)^{-1} \in \Gamma(x)\),
    and such \(\mcal{G}_0\) would therefore be block-lower-triangular with
    diagonal entries such that the expression
    \begin{align*}
            \mcal{O}_L (\mcal{Z}^\top)^\top
            \begin{bmatrix}
                \mcal{H}_L (x) \\
                & \ddots \\
                & & \mcal{H}_L (x)
            \end{bmatrix}
            \underbrace{
            \begin{bmatrix}
                G_0 ^\star (I + D_0)^{-1} \\
                \vdots & \ddots \\
                \star & \cdots & G_{L - 1} ^\star (I + D_{L - 1})^{-1}
            \end{bmatrix}}_{\mcal{G}^\star (I + \mcal{D})^{-1}}
    \end{align*}
    is block-lower triangular with identity diagonals.
    The block-lower triangular result similarly holds for \(\mcal{H}_L (u)\)
    in the second term, without the requirement of identity diagonals.
    This demonstrates that \(\mcal{G}_0\) satisfies the algebraic requirements
    to be a solution for \eqref{eqn:robust-data-sls-lqr},
    and therefore induces valid approximate system responses
    \(\hat{\Phi}_x, \hat{\Phi}_u\) from data.
    
    From~\cite{elkies2011bound}
    upper-triangular matrices of all \(1\)'s are norm-bounded via
    \begin{align*}
        \norm{U_L}_2
        = \frac{1}{2 \sin (\pi / (4L + 2))}
        \leq \frac{2 L + \log L}{\pi},
        \quad \text{for all \(L \geq 3\)}.
    \end{align*}
    Consequently, \((I + D_k)^{-1}\) exists if
    \(\norm{D_k}_2 < 1\),
    a sufficient condition being
    \begin{align*}
        \norm{\mcal{W}_{[0, T-L]} G_k ^\star}_2
        &= \norm{\begin{bmatrix} I & 0 & \cdots & 0 \end{bmatrix}
                (I_L \otimes \mcal{H}_L (w))
                (U_L \otimes I_n)
                G_k ^\star}_2 \\
        &\leq 1 \cdot \norm{\mcal{H}_L (w)}_2 \cdot \norm{U}_L \cdot \norm{G_k ^\star}_2 \\
        &\leq \varepsilon \cdot \parens{\frac{2 L + \log L}{\pi}} \cdot \norm{G_k ^\star}_2 \\
        &\leq \sqrt{\varepsilon}
    \end{align*}
    via the norm equality \(\norm{A \otimes B}_2 = \norm{A}_2 \cdot \norm{B}_2\).
    This results in each \(\norm{D_k}_2 \leq 1/\sqrt{\varepsilon}\),
    and consequently
    \(\lVert (I + \mcal{D})^{-1} \rVert_2 \leq (1 - \sqrt{\varepsilon})^{-1}\)
    by dominating the inverse of each block diagonal.
    
    Furthermore, feasibility for \eqref{eqn:robust-data-sls-lqr} suffices with
    \begin{align*}
        \norm{\Delta_0}_2
            &= \norm{\mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{H}_L (w)) \mcal{G}_0}_2 \\
            &\leq \sqrt{L} \cdot \norm{\mcal{H}_L (w)}_2 \cdot \norm{\mcal{G}^\star}_2
                \cdot \lVert (I + \mcal{D})^{-1} \rVert_2 \\
            &\leq \sqrt{L} \cdot \varepsilon \cdot \norm{\mcal{G}^\star}_2 \cdot \frac{1}{1 - \sqrt{\varepsilon}} \\
            &< \sqrt{\varepsilon} L = \gamma_0 < 1
    \end{align*}
    
    
\end{proof}

This concludes the first part of the sub-optimality proof:
modifying a \(\mcal{G}^\star\) that is optimal on
problem \eqref{eqn:robust-data-sls-lqr} with noiseless data,
into a \(\mcal{G}_0\) that is feasible on
problem \eqref{eqn:robust-data-sls-lqr} with noisy data.
This is readily applicable in the sub-optimality proof,
presented below.

\begin{theorem}
    \label{thm:subopt}
    Let \(\hat{\mcal{G}}, \hat{\gamma}\) be the optimal solution to
    \eqref{eqn:robust-data-sls-lqr};
    let \(\mcal{G}^\star\) be the optimal LQR cost derived from noiseless data \(z, u\),
    such that \(\mcal{G}_0, \gamma_0\) as defined in Lemma~\ref{lem:feas-soln}
    is a feasible solution to \eqref{eqn:robust-data-sls-lqr};
    let \(\hat{J}\) be the LQR cost induced by \(\hat{\mcal{G}}\)
    on the true system,
    and \(J^\star\) be the LQR cost induced by \(\mcal{G}^\star\).
    The relative error of sub-optimality is then
    \begin{align*}
        \frac{\hat{J} - J^\star}{J^\star} \leq 4 \sqrt{\varepsilon} (L + 1)
    \end{align*}
    provided \(\gamma_0 = \sqrt{\varepsilon} L < 1/2\).
\end{theorem}
\begin{proof}
    From the derivation of \eqref{eqn:robust-data-sls-lqr},
    the cost of \(\hat{\mcal{G}}\) on the true dynamics is upper-bounded via
    \begin{align*}
        \hat{J}
            = \sigma \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
            \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}
            (I + \Delta)^{-1}}_F
        \leq \frac{\sigma}{1 - \hat{\gamma}}
        \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
            \begin{bmatrix} \hat{\Phi}_x \\ \hat{\Phi}_u \end{bmatrix}}_F
    \end{align*}
    where the RHS is the optimal value of \eqref{eqn:robust-data-sls-lqr}.
    By the optimality of \(\hat{\gamma}, \hat{\mcal{G}}\),
    this means that any other \(\gamma_0, \mcal{G}_0\) would achieve a higher cost of
    \begin{align*}
        &\leq \frac{\sigma}{1 - \gamma_0}
            \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
            \begin{bmatrix}
                \mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{H}_L (x)) \\
                \mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{H}_L (u))
            \end{bmatrix}
            \mcal{G}_0}_F \\
        &= \frac{\sigma}{1 - \gamma_0}
            \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
            \begin{bmatrix}
                \Phi_x ^\star \\ \Phi_u ^\star
            \end{bmatrix}
            (I + \mcal{D})^{-1}}_F \\
        &\leq \frac{\sigma}{(1 - \gamma_0) (1 - \sqrt{\varepsilon})}
            \norm{\begin{bmatrix} \mcal{Q}^{1/2} \\ & \mcal{R}^{1/2} \end{bmatrix}
            \begin{bmatrix}
                \Phi_x ^\star \\ \Phi_u ^\star \end{bmatrix}}_F \\
        &= \frac{J^\star}{(1 - \gamma_0) (1 - \sqrt{\varepsilon})}
    \end{align*}
    where we use the relations
    \begin{align*}
        \mcal{G}_0 = \mcal{G}^\star (I + \mcal{D})^{-1},
        \quad
        \begin{bmatrix} \Phi_x ^\star \\ \Phi_u ^\star \end{bmatrix}
        = \begin{bmatrix}
            \mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{H}_L (x)) \\
            \mcal{O}_L (\mcal{Z}^\top)^\top (I_L \otimes \mcal{H}_L (u))
        \end{bmatrix} \mcal{G}^\star,
        \quad
        \norm{(I + \mcal{D})^{-1}}_2 \leq \frac{1}{1 - \sqrt{\varepsilon}}
    \end{align*}
    Simplifying the algebra above yields
    \begin{align*}
        \frac{J - J^\star}{J^\star}
            \leq \frac{\gamma_0 + \sqrt{\varepsilon} - \gamma_0 \sqrt{\varepsilon}}
                    {(1 - \gamma_0) (1 - \sqrt{\varepsilon})}
    \end{align*}
    Because \(\gamma_0 = \sqrt{\varepsilon L \norm{\mcal{G}^\star}} \leq 1/2\)
    and \(\sqrt{\varepsilon} \leq 1/2\),
    the inequality simplifies as
    \begin{align*}
        \frac{\gamma_0 + \sqrt{\varepsilon} - \gamma_0 \sqrt{\varepsilon}}
                    {(1 - \gamma_0) (1 - \sqrt{\varepsilon})}
        \leq 4 \parens{\sqrt{\varepsilon L \norm{\mcal{G}^\star}_2} + \sqrt{\varepsilon}}
        \leq 4 \sqrt{\varepsilon} \parens{\sqrt{L \norm{\mcal{G}^\star}_2} + 1}
    \end{align*}
\end{proof}


==> 05-sample-comp.tex <==
\section{Sample Complexity}
\label{sec:sample-comp}

In this section we examine the sample complexity of using a
data-driven approach: how many samples are needed
to guarantee both feasibility and performance?
The crux of this is the analysis
of the noise Hankel matrix \(\mcal{H}_L (w)\),
whose norm affects controller performance.
We first review some results from high-dimensional statistics
before proceeding with a norm concentration analysis of
\(\mcal{H}_L (w)\),
followed by sample complexity results.



% In this section we first review some facts from high-dimensional statistics
% on the norm concentration of sub-Gaussian vectors.
% Since each \(n\)-dimensional component \(w(t) \sim \mcal{N}(0, \sigma^2 I)\),
% it is valid to view \(w\) as an \(nT\)-dimensional sub-Gaussian vector.
% Indeed, we then present a decomposition of \(\mcal{H}_L (w)\)
% that isolates \(w\) as a vector.
% Next, since linear systems enjoy a superposition property:
% the superposition and also \emph{averaging} of process noise
% across trajectories allows us to reduce variance --- for which
% we can calculate a lower bound on the number of independent trajectory \(x, u\)
% samples necessary to achieve the performance described earlier in the paper.



\subsection{A Review of High Dimensional Statistics}
A number of results readily follow from
high-dimensional statistics~\cite{rigollet2015high},
which we supply without proof.

\begin{definition}
    Write \(X \sim \textrm{subG}(\sigma^2)\)
    to mean that \(X \in \mbb{R}\) is a sub-Gaussian
    random variable with parameter \(\sigma^2\).
    Such \(X\) satisfies \(\mbb{E}[X] = 0\)
    and has a moment generating function bounded by
    \begin{align*}
        \E [\exp(tX)] \leq \exp \parens{\frac{t^2 \sigma^2}{2}},
        \qquad \text{for all \(t \in \mbb{R}\)}
    \end{align*}
\end{definition}
By extension, we say that a vector
\(X \in \mbb{R}^{d}\)
is sub-Gaussian with parameter \(\sigma^2\)
if each component \(X(k) \sim \trm{subG}(\sigma^2)\).
By construction, this means that \(w \in \mbb{R}^d\)
is a sub-Gaussian random vector of dimension \(d = nT\).

\begin{lemma}
    \label{lem:norm-conc}
    Let \(X \in \mbb{R}^d\) be a sub-Gaussian random vector
    with parameter \(\sigma^2\). Then
    \begin{align*}
        \E \big[\max_{\theta \in \mcal{B}_d} \theta^\top X \big]
        = \E \big[\max_{\theta \in \mcal{B}_d} \lvert \theta^\top X \rvert \big]
        \leq 4 \sigma \sqrt{d}
    \end{align*}
    where \(\mcal{B}_d\) is the unit \(\ell^2\) ball in \(\mbb{R}^d\).
    Moreover, for any \(\delta > 0\), then with probability \(1 - \delta\),
    \begin{align*}
        \max_{\theta \in \mcal{B}_d} \theta^\top X
        = \max_{\theta \in \mcal{B}_d} \lvert \theta^\top X \rvert
        \leq 4 \sigma \sqrt{d} + 2 \sigma \sqrt{2 \log (1 / \delta)}
    \end{align*}
\end{lemma}
For fixed \(X \in \mbb{R}^d\),
maximizing \(\theta^\top X\) is equivalent to \(\norm{X}_2\)
because the optimal value of \(\theta\) is attained at \(\theta = X / \norm{X}_2\).


\subsection{Analysis}
The analysis of \(\mcal{H}_L (w)\) is readily adapted into the
results from high-dimensional statistics.

\begin{lemma}
    \label{lem:Hw-bound}
    Let \(w \in \mbb{R}^{nT}\) be such that  \(w \sim \trm{subG}(\sigma^2)\), then
    \begin{align*}
    \norm{\mcal{H}_L (w)}_2
        \leq 4 \sigma T \sqrt{n} + 2 \sigma \sqrt{2 T \log (1/\delta)}
    \end{align*}
\end{lemma}
\begin{proof}
    We may decompose \(\mcal{H}_L (w)\) as
    \begin{align*}
        \mcal{H}_L (w)
            = \begin{bmatrix} P_0 & P_1 & \cdots & P_{T - L} \end{bmatrix}
                (I_{T - L + 1} \otimes w)
    \end{align*}
    where each \(P_k \in \mbb{R}^{nL \times nT}\)
    is a matrix that projects out the \(w_{[k, k+L-1]} \in \mbb{R}^{nL}\)
    segment of \(w\).
    The concentration bound from Lemma~\ref{lem:norm-conc} therefore implies that
    \begin{align*}
        \norm{w}_2 \leq 4 \sigma \sqrt{nT} + 2 \sigma \sqrt{2 \log (1 / \delta)}
    \end{align*}
    with probability \(1 - \delta\).
    As each \(\norm{P_k}_2 = 1\),
    the block matrix of horizontal projectors then has norm
    \begin{align*}
        \norm{\begin{bmatrix} P_0 & P_1 & \cdots & P_{T - L} \end{bmatrix}}_2
        \leq \sqrt{T - L + 1}
        \leq \sqrt{T}
    \end{align*}
    Applying sub-multiplicativity of the spectral norm concludes the proof.
\end{proof}

Up until now we have made the implicit assumption that
\(\norm{\mcal{H}_L (w)}_2 \leq \varepsilon\) is small.
Indeed this is possible by taking \emph{multiple} trajectory samples.
By the superposition property of linear systems,
the linear combination of different trajectories
\(\{x^{(i)}, u^{(i)}, w^{(i)}\}_{i = 1}^{N}\) remains valid.
That is, each \(x^{(i)}, u^{(i)}, w^{(i)}\) will satisfy
the system dynamics, as formulated in \eqref{eqn:data-only-constr}.
Consequently, we may use the averages
\begin{align*}
    x = \frac{1}{N} \sum_{i = 1}^{N} x^{(i)},
    \qquad
    u = \frac{1}{N} \sum_{i = 1}^{N} u^{(i)},
    \qquad
    w = \frac{1}{N} \sum_{i = 1}^{N} w^{(i)},
\end{align*}
to construct the Hankel matrices \(\mcal{H}_L (x), \mcal{H}_L (u), \mcal{H}_L (w)\)
used in the optimization problem and analysis.
In particular, this means that now
\(w \sim \trm{subG}(\sigma^2 / N)\).

\begin{theorem}
    Suppose that each \(w^{(i)} (t) \sim \mcal{N}(0, \sigma^2 I)\),
    and the averaged noise vector \(w\) be as above.
    To achieve \(\norm{\mcal{H}_L (w)}_2 \leq \varepsilon\)
    with at least probability \(1 - \delta\),
    a sufficient number of samples is
    \begin{align*}
        N \geq \frac{16 \sigma^2 T^2 n}{\varepsilon^2} + \frac{8 \sigma^2 T \log(1/\delta)}{\varepsilon^2}
    \end{align*}
\end{theorem}
\begin{proof}
    Substituting in the new variance \(\sigma / \sqrt{N} \mapsto \sigma\)
    for Lemma~\ref{lem:Hw-bound} such that
    \begin{align*}
        \frac{4 \sigma T \sqrt{n}}{\sqrt{N}}
            + \frac{2 \sigma \sqrt{2 T \log (1 / \delta)}}{\sqrt{N}}
            \leq \varepsilon
    \end{align*}
    and solving for \(N\),
    \begin{align*}
        \frac{4 \sigma T \sqrt{n}}{\varepsilon}
            + \frac{2 \sigma \sqrt{2 T \log(1 / \delta)}}{\varepsilon}
            \leq \sqrt{N}
    \end{align*}
    Using the algebraic inequality \(2a^2 + 2b^2 \geq (a + b)^2\)
    yields the desired result.
\end{proof}
It's important to point out that this bound is rather conservative:
experimentally it is the case that significantly less samples
suffice to achieve a high-probability guarantee.
As a remark, a number of result in concentration of norm
do exist for random matrices~\cite{tropp2012user},
but tend to give laxer bounds as they do not sufficiently exploit problem structure.


==> lipschitz-concentration.tex <==
 We then immediately have the following result, which follows from the concentration of Lipschitz functions of Gaussian random variables, e.g., Theorem 2.26 of \cite{wainwright2019high}.

\begin{lemma} \label{lem:hankel-bound}
Let $\bar w_{[-1,T-2]}$ be defined as in equation \eqref{eq:averages}.  Then
\begin{equation}
    \mathbb P\left[\twonorm{\mcal H_L(\bar w)}\geq t + \frac{\sigma T}{\sqrt{N}}\right] \leq e^{-\frac{t^2 N}{\sigma^2 T}}
\end{equation}
for all $t \geq 0$.
\end{lemma}
\begin{proof}
Note that 
\begin{multline*}
    \mcal{H}_L (\bar w)
            = \begin{bmatrix} P_0 & P_1 & \cdots & P_{T - L} \end{bmatrix}
                (I_{T - L + 1} \otimes \bar w) \\ \ed\frac{\sigma}{\sqrt{N}} \begin{bmatrix} P_0 & P_1 & \cdots & P_{T - L} \end{bmatrix}
                (I_{T - L + 1} \otimes v) =: \mcal{\bar H}_L(v),
\end{multline*}
where $v\sim{}\mathcal{N}(0,I_{T})$.  Noting that $\twonorm{\begin{bmatrix} P_0 & P_1 & \cdots & P_{T - L} \end{bmatrix}}\leq \sqrt{T-L+1}\leq \sqrt{T}$ and applying the reverse triangle inequality, we conclude that $\twonorm{\mcal{\bar H}_L(v)}$ is a $\sigma\sqrt{\frac{T}{N}}$-Lipschitz function of $v$.  Finally, observe that
\[
\mathbb E\frac{\sigma}{\sqrt{N}} \twonorm{\begin{bmatrix} P_0 & P_1 & \cdots & P_{T - L} \end{bmatrix}
                (I_{T - L + 1} \otimes v)} \leq \sigma \sqrt{\frac{T}{N}}\mathbb E \twonorm{v} \leq \frac{\sigma T}{\sqrt{N}},
\]
where the final inequality follows from $\mathbb E \twonorm{v}\leq \sqrt{T}$ for $v\sim{}\mathcal{N}(0,I_{T})$.
The result then follows immediately by the one-sided version of Theorem 2.26 of \cite{wainwright2019high}.
\end{proof}

Combining Lemma \ref{lem:hankel-bound} and Theorem \ref{thm:subopt}, we obtain the following end-to-end sample-complexity bound.
\begin{corollary}
Assume that $T \geq \log(1/\delta)$.  Then if
\begin{equation}\label{eq:n-bound}
N \geq \sigma^2\max(36T^2\twonorm{\mcal G^\star}^2L,16\twonorm{\mcal G^\star}^2\twonorm{\mcal T_{T-L+1}(I)}^2T),
\end{equation}
we have with probability at least $1-\delta$ that
\begin{equation}
    \frac{\hat J - J^\star}{J^\star} \leq
    6\frac{T\sigma}{\sqrt{N}}\left(2\twonorm{\mcal G^\star}\sqrt{ L} + \frac{\norm{\mcal{T}_{T - L + 1} (I)}_2\norm{\mcal G^\star}_2}{\sqrt{T}} + 2\twonorm{\mcal Q^{1/2}}\twonorm{\mcal G^{\star}}\twonorm{\mcal T_{T-L+1}(I)}/J^\star\right)
\end{equation}
\end{corollary}
\begin{proof}
Inverting the probability bound from Lemma \ref{lem:hankel-bound}, we have that with probability at least $1-\delta$ that
\[
\twonorm{\mcal H_L(\bar w)}\leq \frac{\sigma T}{\sqrt{N}} + \sigma\sqrt{\frac{T\log(1/\delta)}{N}} \leq \frac{2T\sigma}{\sqrt{N}},
\]
where the final inequality follows from the assumption on $T\geq \log(1/\delta)$. There, we have that the bounds \eqref{eq:eps-bound} are satisfied if the conditions \eqref{eq:n-bound} are met, proving the result by combining the above bound with Theorem \ref{thm:subopt}.
\end{proof}
